Functional Latent Dynamics for Irregularly Sampled Time Series Forecasting

Irregularly sampled time series with missing values are often observed in multiple real-world applications such as healthcare, climate and astronomy. They pose a significant challenge to standard deep learning models that operate only on fully observed and regularly sampled time series. In order to capture the continuous dynamics of the irregular time series, many models rely on solving an Ordinary Differential Equation (ODE) in the hidden state. These ODE-based models tend to perform slow and require large memory due to sequential operations and a complex ODE solver. As an alternative to complex ODE-based models, we propose a family of models called Functional Latent Dynamics (FLD). Instead of solving the ODE, we use simple curves which exist at all time points to specify the continuous latent state in the model. The coefficients of these curves are learned only from the observed values in the time series ignoring the missing values. Through extensive experiments, we demonstrate that FLD achieves better performance compared to the best ODE-based model while reducing the runtime and memory overhead. Specifically, FLD requires an order of magnitude less time to infer the forecasts compared to the best performing forecasting model.

==> content/02_Problem-Formulation.tex <==
\newcommand{\obs}{^\text{obs}} \newcommand{\R}{\mathbb{R}}
\newcommand{\nan}{\text{NaN}}
\section{Problem Formulation}
An \emph{irregularly sampled multivariate time series} (IMTS) is a sequence $X =
[(t_1,v_1),(t_2,v_2),\ldots,(t_N,v_N)]$, where $v_n \in (\mathbb{R} \cup
\{\text{NaN}\}) ^C$ is the \emph{observation} at \emph{time} $t_n \in
\mathbb{R}$ for all $n \in \{1,\dots, N\}$ and $C \in \mathbb{N}$ represents the number of
\emph{channels}. NaN represents the occurrence of a missing observation. 
Given an IMTS $X$, \emph{an unobserved forecasting target} for $X$ is a sequence 
$u := (u_1, u_2, \ldots, u_K) \in \mathbb{R}^{K}$, where $u_k
> t_n$ for all $i \in \{1,\dots,K\}$ and $j \in \{1,\dots,N\}$. 

The task of IMTS forecasting involves predicting the \emph{forecasting targets}
$y := (y_1, y_2, \ldots, y_K)$ with $y_k \in (\mathbb{R} \cup \{\text{NaN}\})
^C$ being the target for query time $u_k$. Given the output of a forecasting
model $\hat{y_1}, \hat{y_2}, \ldots, \hat{y_K}$ the forecasting objective is to
minimize
\begin{align*}
    \sum_{\substack{i=1,\dots,K \\ c=1,\dots,C \\ y_{i,c}\neq \text{NaN}}}\ell(y_{i,c} , \hat{y}_{i,c}),
\end{align*} with $\ell : \mathbb{R}^{2} \to \mathbb{R}$ being an arbitrary scalar loss function. 
